Runners in action

Runners of algebraic effects, also known as comodels, provide a mathematical model of resource management. We show that they also give rise to a programming concept that models top-level external resources, as well as allows programmers to modularly define their own intermediate "virtual machines". We capture the core ideas of programming with runners in an equational calculus $\lambda_{\mathsf{coop}}$, which we equip with a sound and coherent denotational semantics that guarantees the linear use of resources and execution of finalisation code. We accompany $\lambda_{\mathsf{coop}}$ with examples of runners in action, provide a prototype language implementation in OCaml, as well as a Haskell library based on $\lambda_{\mathsf{coop}}$.

==> coop.tex <==
% !TEX root = runners-in-action.tex

\lstdefinelanguage{coop}{
    backgroundcolor=\color{white},
    basicstyle={\small\sffamily},
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    columns=fullflexible,
    commentstyle=\color{codepurple},
    identifierstyle={\sffamily},
    keepspaces=true,
    keywordstyle=[1]{\color{keywordColor}},
    mathescape=true,
    numbers=none,
    numbersep=5pt,
    numberstyle=\tiny\color{codegray},
    rulecolor=\color{lightgray},
    sensitive=true,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    stringstyle=\color{codepurple},
    tabsize=2,
    texcl=true,
    xleftmargin=1em,
    xrightmargin=1em,
    morekeywords=[1]{
     @,
     and,
     any,
     as,
     bool,
     cohandler,
     do,
     else,
     empty,
     end,
     external,
     finally,
     fun,
     getenv,
     setenv,
     handle,
     handler,
     if,
     in,
     initially,
     int,
     kernel,
     kill,
     let,
     load,
     match,
     of,
     operation,
     raise,
     rec,
     return,
     run,
     runner,
     signal,
     string,
     then,
     try,
     to,
     type,
     unit,
     use,
     user,
     using,
     val,
     with
    },
    morecomment=[n]{(*}{*)},
    morestring=[b]",
    literate={->}{$\rightarrow\,$}{1}
                {>>=}{\footnotesize$\mathtt{\blue{\boldsymbol>\boldsymbol>\boldsymbol=}}$}{1}
                {;}{$\boldsymbol;$}{1}
                {++}{$+\!\!+$}{1}
%                {finally}{{\bfseries\color{NavyBlue}finally}}{1}
%                {using}{{\bfseries\color{NavyBlue}using}}{1}
%                {run}{{\bfseries\color{NavyBlue}run}}{1}
%                {runner}{{\bfseries\color{NavyBlue}runner}}{1}
%                {if}{{\bfseries\color{NavyBlue}if}}{1}
%                {then}{{\bfseries\color{NavyBlue}then}}{1}
%                {else}{{\bfseries\color{NavyBlue}else}}{1}
%                {let}{{\bfseries\color{NavyBlue}let}}{1}
%                {in}{{\bfseries\color{NavyBlue}in}}{1}
%                {try}{{\bfseries\color{NavyBlue}try}}{1}
%                {with}{{\bfseries\color{NavyBlue}with}}{1}
%                {raise}{{\bfseries\color{NavyBlue}raise}}{1}
                ,
    frame=single
}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "runners-in-action"
%%% End:

